BoostMVSNeRFs: Boosting MVS-based NeRFs to Generalizable View Synthesis in Large-scale Scenes

While Neural Radiance Fields (NeRFs) have demonstrated exceptional quality, their protracted training duration remains a limitation. Generalizable and MVS-based NeRFs, although capable of mitigating training time, often incur tradeoffs in quality. This paper presents a novel approach called BoostMVSNeRFs to enhance the rendering quality of MVS-based NeRFs in large-scale scenes. We first identify limitations in MVS-based NeRF methods, such as restricted viewport coverage and artifacts due to limited input views. Then, we address these limitations by proposing a new method that selects and combines multiple cost volumes during volume rendering. Our method does not require training and can adapt to any MVS-based NeRF methods in a feed-forward fashion to improve rendering quality. Furthermore, our approach is also end-to-end trainable, allowing fine-tuning on specific scenes. We demonstrate the effectiveness of our method through experiments on large-scale datasets, showing significant rendering quality improvements in large-scale scenes and unbounded outdoor scenarios. We release the source code of BoostMVSNeRFs at https://su-terry.github.io/BoostMVSNeRFs/.

==> tables/quantitative_llff.tex <==
\begin{table}[t]
\centering
\small
\hai{Suppl.}
\caption{\textbf{Quantitative comparisons with state-of-the-art methods on the LLFF~\cite{mildenhall2019local} dataset.}}
\label{tab:quantitative_llff}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method & Setting & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
MVSNeRF~\cite{chen2021mvsnerf} & \multirow{4}{*}{\makecell{No per-scene\\optimization}} & 21.65 & 0.719 & 0.226 \\
% NeRFusion~\cite{zhang2022nerfusion} & \\
PointNeRF~\cite{xu2022point} \\
SurfelNeRF~\cite{gao2023surfelnerf} \\
% MVSNeRF~\cite{chen2021mvsnerf} &  & \\
% MVSNeRF~\cite{chen2021mvsnerf} + Ours &  & \\
% ENeRF~\cite{lin2022efficient} &  & 23.10 & 0.827 & 0.190 \\
% ENeRF~\cite{lin2022efficient} + Ours &  & \\
Ours &  & 23.41 & 0.836 & 0.184 \\
\midrule
F2-NeRF~\cite{wang2023f2} & \multirow{5}{*}{\makecell{Per-scene\\optimization}} \\
Zip-NeRF~\cite{barron2023zip} & & 26.18 & 0.803 & 0.169 \\
$\text{MVSNeRF}_\text{ft}$~\cite{chen2021mvsnerf} & & \\
% $\text{NeRFusion}_\text{ft}$~\cite{zhang2022nerfusion} \\
$\text{PointNeRF}_\text{ft}$~\cite{xu2022point} \\
$\text{SurfelNeRF}_\text{ft}$~\cite{gao2023surfelnerf} \\
% $\text{MVSNeRF}_\text{ft}$~\cite{chen2021mvsnerf} &  & \\
% MVSNeRF~\cite{chen2021mvsnerf} + $\text{Ours}_\text{ft}$ &  & \\
% $\text{ENeRF}_\text{ft}$~\cite{lin2022efficient} &  & \\
% ENeRF~\cite{lin2022efficient} + $\text{Ours}_\text{ft}$ &  & \\
$\text{Ours}_\text{ft}$ &  & 24.70 & 0.866 & 0.148 \\
\bottomrule
\end{tabular}%
% }
\end{table}

==> tables/quantitative_sparse_scannet.tex <==

\begin{table}[t]
% \hai{PointNeRF fails for 3 scenes, plz refer to the supplementary.}
\centering
\small
\caption{\textbf{Quantitative comparisons with state-of-the-art methods on the ScanNet~\cite{dai2017scannet} dataset with sparse input.}
*: F2-NeRF fails at subspace division processing in 4 out of 8 scenes on the ScanNet dataset. Therefore, we average the metrics among the scenes that succeed.}
% \vspace{-3mm}
\label{tab:quantitative_scannet}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method & Setting & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
MVSNeRF~\cite{chen2021mvsnerf} & \multirow{3}{*}{\makecell{No per-scene\\optimization}} & 19.13 & 0.737 & 0.431 \\
% NeRFusion~\cite{zhang2022nerfusion}* & & - & - & - \\
% PointNeRF~\cite{xu2022point}* & & - & - & - \\
SurfelNeRF~\cite{gao2023surfelnerf} & & 20.20 & 0.605 & 0.521 \\
% MVSNeRF~\cite{chen2021mvsnerf} &  & \\
% MVSNeRF~\cite{chen2021mvsnerf} + Ours &  & \\
% ENeRF~\cite{lin2022efficient} &  & \\
% ENeRF~\cite{lin2022efficient} + Ours &  & \\
Ours &  & \textbf{24.22} & \textbf{0.868} & \textbf{0.361}   \\
\midrule
F2-NeRF*~\cite{wang2023f2} & \multirow{5}{*}{\makecell{Per-scene\\optimization}} & 11.88 & 0.585 & 0.696 \\
$\text{MVSNeRF}_\text{ft}$~\cite{chen2021mvsnerf} & & 21.16 & 0.768 & 0.412 \\
% $\text{NeRFusion}_\text{ft}$~\cite{zhang2022nerfusion}* & & - & - & - \\
% $\text{PointNeRF}_\text{ft}$~\cite{xu2022point}* & & 24.85* & 0.859* & 0.350* \\
$\text{SurfelNeRF}_\text{ft}$~\cite{gao2023surfelnerf} & & 18.67 & 0.563 & 0.560 \\
Zip-NeRF~\cite{barron2023zip} & & 14.69 & 0.481 & 0.658 \\
% $\text{MVSNeRF}_\text{ft}$~\cite{chen2021mvsnerf} &  & \\
% MVSNeRF~\cite{chen2021mvsnerf} + $\text{Ours}_\text{ft}$ &  & \\
% $\text{ENeRF}_\text{ft}$~\cite{lin2022efficient} &  & \\
% ENeRF~\cite{lin2022efficient} + $\text{Ours}_\text{ft}$ &  & \\
$\text{Ours}_\text{ft}$ &  & \textbf{25.06} & \textbf{0.877} & \textbf{0.336} \\
\bottomrule
\end{tabular}%
}
\end{table}
